OncoNet: Weakly Supervised Siamese Network to automate cancer treatment response assessment between longitudinal FDG PET/CT examinations

FDG PET/CT imaging is a resource intensive examination critical for managing malignant disease and is particularly important for longitudinal assessment during therapy. Approaches to automate longtudinal analysis present many challenges including lack of available longitudinal datasets, managing complex large multimodal imaging examinations, and need for detailed annotations for traditional supervised machine learning. In this work we develop OncoNet, novel machine learning algorithm that assesses treatment response from a 1,954 pairs of sequential FDG PET/CT exams through weak supervision using the standard uptake values (SUVmax) in associated radiology reports. OncoNet demonstrates an AUROC of 0.86 and 0.84 on internal and external institution test sets respectively for determination of change between scans while also showing strong agreement to clinical scoring systems with a kappa score of 0.8. We also curated a dataset of 1,954 paired FDG PET/CT exams designed for response assessment for the broader machine learning in healthcare research community. Automated assessment of radiographic response from FDG PET/CT with OncoNet could provide clinicians with a valuable tool to rapidly and consistently interpret change over time in longitudinal multi-modal imaging exams.

==> figures.tex <==
% !TEX root = main.tex

\thispagestyle{empty}

\begin{figure}
\centering
{\spacing{1}\fontsize{7}{8}\selectfont
\includegraphics[width=\textwidth]{FIG/FIG1/figure_1.pdf}
\caption{
\textbf{\added{Weak supervision, multi-task learning, and spatial attention are combined to  build convolutional neural networks (CNNs) for FDG-PET/CT analysis without hand-labeled training data.}}
%
\textbf{(a)} Our dataset of $8,144$ FDG-PET/CT examinations. Each exam consists of (1) a 3D scan consisting of approximately 250 FDG-PET and CT slices and (2) a natural language, unstructured report written by the interpreting radiologist at the time of the study. Critically, there are no structured, ground truth labels for metabolic abnormalities in each anatomical region.
%
\textbf{(b)} Tagging functions powered by regular expressions extract sentences that mention anatomical regions.  
%
\textbf{(c)} A language model predicts whether there is a metabolic abnormality in the tagged anatomical region. 
%
\textbf{(d)} Conflicting language model predictions are reconciled into one probability of abnormality for each region. This is done by propagating probabilities up the directed acyclic graph of the ontology. 
%
\textbf{(e)} The entire whole-body PET/CT scan is encoded using a 3D-convolutional neural network. This encoding process produces a three-dimensional representation of the original scan. 
%
\textbf{(f)} Each task head uses an attention module to extract from the encoded scan the voxels most relevant to the anatomical region it is charged with. We apply a final linear classification layer to weighted-sum of those voxels to make a final binary prediction for each region. To train the scan model, we minimize the cross-entropy loss between the report model predictions (left) and the scan model predictions (right). 
}\label{fig:overview}}
\end{figure}

\clearpage
\thispagestyle{empty}

\begin{figure}
\centering
{\spacing{1}\fontsize{7}{8}\selectfont
\includegraphics[width=\textwidth]{FIG/FIG2/figure_2.pdf}
\caption{
\textbf{\added{Combining weakly supervised multi-task learning with spatial attention mechanisms  enables  automated  abnormality  detection and \del{localization} \add{location estimation} in  FDG-PET/CT.}}
%
\textbf{(a)} Our model's predictive performance across anatomical regions. Each bar indicates the model's AUROC for detecting abnormal metabolic activity in a particular anatomical region. Confidence intervals ($95\%$) \addc{about the mean} were determined using bootstrapping over $n=5$ random seeds. The individual AUROC result for each initialization is shown as a blue dot. Anatomical regions are sorted in order of increasing mean AUROC. 
%
\textbf{(b-d)} Sensitivity curve for abnormality detection in the \textbf{(b)} chest, \textbf{(c)} liver, and \textbf{(d)} inguinal lymph nodes. Each point on the curve indicates the sensitivity of our model at a prediction threshold where $x\%$ of the exams in our test set are flagged as abnormal. The sensitivity curve of a perfect detector \added{(i.e. a model that ranks all abnormal examples above all normal examples)} is shown in grey. The shaded region represents confidence intervals ($95\%$) \addc{about the mean} computed using bootstrapping over $n=5$ random seeds. The sensitivity curves for each of those initializations are shown in light \added{(b) green, (c) yellow, and (d) pink}. Sensitivity curves illustrate the utility of the model in a potential screening application. With our model, clinicians could ignore around $15\%$ of exams while maintaining $99\%$ sensitivity in liver abnormality screening.
%
\textbf{(e)} 3D saliency map for abnormality detection in the chest (green), liver (pink), and inguinal lymph nodes (yellow). Colored volumes indicate regions where small perturbations to the input scan most effect the model's prediction for chest, liver, and inguinal lymph nodes.  
}\label{fig:case-studies}}
\end{figure}

\clearpage
\thispagestyle{empty}

\begin{figure}
\centering
{\spacing{1}\fontsize{7}{8}\selectfont
\includegraphics[width=\textwidth]{FIG/FIG3/figure_3.pdf}
\caption{
\textbf{\added{Weak supervision reduces labeling costs for automated abnormality detection and \del{localization} \add{location estimation}.}}
\textbf{(a)} Our labeling framework outperforms a regular expression baseline on 24 of the 26 regions specified in our test set. The five dots for each region represent the difference in F1-score between the baseline and our labeling framework for five different random seeds. For each region, we also show the average difference across $n=5$ seeds and 95\% confidence intervals computed via bootstrapping. 
%
\textbf{(b)}   26-region abnormality \del{localization} \add{detection} models trained on large datasets using weak supervision outperform models fully-supervised on a small dataset.\R{2R_1_8_start} We compare three models: (yellow, left) a fully supervised model trained using \del{$n=400$} \add{$391$} manually annotated training examples, (blue, middle) a weakly supervised model trained using $6,530$ automatically annotated training examples, and (green, right) a hybrid model trained using a combined dataset of \del{$n=6,930$} \add{$6,921$} training examples, \del{$n=400$} \add{$391$}of which are manually annotated\R{2R_1_8_end}. To the left, we show the distribution of AUROC across all 26 regions and 5 random seeds. Each point represents the AUROC on one region and one random seed. \addc{Bars represent mean AUROC across $n=26$ regions and $5$ random seeds.} To the right, we compare the supervision approaches on five representative regions: skeleton, lungs, carinal lymph node, liver, and axillary lymph node. Bars represent mean AUROC across $n=5$ seeds and 95\% confidence intervals computed via bootstrapping. The numbers for all regions are provided in Supplementary Table 3.
%
\textbf{(c)} Binary abnormality detection AUROC vs. the number of training data points. The performance of our weakly supervised model is statistically equivalent to that of a traditionally supervised baseline model (trained using summary codes) ( $p = 0.1933$ paired permutation test). The shape of the curve suggests that more data, which can be rapidly annotated using our framework, would lead to a continued increase in performance. Line shows the mean AUROC across $n=5$ random seeds and shaded regions represent 95\% confidence intervals computed via bootstrapping. 
%
}\label{fig:weak-supervision}}
\end{figure}

\begin{figure}
\centering
{\spacing{1}\fontsize{7}{8}\selectfont
\includegraphics[width=\textwidth]{FIG/FIG4/figure_4.pdf}
\caption{
\textbf{\added{Multi-task learning improves automated \del{localization} \add{location estimation} performance, reduces computational cost, and facilitates mortality prediction.}}
\textbf{(a)} Gains from multi-task learning are the greatest in regions with severe class imbalance. For each region, the difference in abnormality \del{localization} \add{detection} AUROC between a multi-task model and a single task model is plotted against the class balance for the region. If a region exhibits class balance 10:1, then for every exam with an abnormality in the region, there will be ten exams where the region is normal. The single-task and multi-task models were both trained on five different random seeds and differences in mean AUROC are plotted.\addc{ We also fit a linear model to the two variables and report Pearson correlation coefficient $r^2=0.808$ and two-sided p-value $p=6.94\times10^{-8}$ computed using the Wald test.} \addc{Shaded regions represent 95\% confidence intervals computed via bootstrapping across $n=30$ regions (\textit{e.g.} pancreas, lungs)}. 
%
\textbf{(b)} Multi-task learning improves performance in regions in which hypermetabolic abnormality is rare. We fine-tune our 26-region multi-task abnormality \del{localization} \add{detection} model to detect abnormalities in four new regions beyond the main 26: celiac lymph nodes, the pancreas, the adrenal gland, and the kidneys. Each of these regions exhibit severe class imbalance with more than 30 positive examples for every negative example. We compare this multi-task approach (right, blue) to two other single task approaches: (teal, left) a single task model pre-trained on Kinetics and (orange, middle) a single task model pre-trained on full-body abnormality detection (in-domain pretraining). Shown for each region and modeling approach is AUROC across $n=5$ random seeds. 95\% confidence intervals about the mean are computed via bootstrapping. 
%
\textbf{(c)} Multi-task model reduces training complexity. We fine-tune our multi-task FDG-PET/CT model in a single-task setting for each of the twenty-six core anatomical regions. We do the same with a model trained on Kinetics \cite{carreira_quo_nodate}, an out-of-domain dataset. The plot shows how mean AUROC across all anatomical regions improves with more epochs of fine-tuning. To the right, we show the best mean AUROC after training to convergence. Confidence intervals ($95\%$) \addc{about the mean} were determined using bootstrapping across $n=5$ random seeds.
%
\added{\textbf{(d)} Multi-task learning improves performance on the task of predicting mortality from FDG-PET/CT scan alone. We frame mortality prediction as a binary classification task, where the model predicts whether the patient’s date of death is within $x$ days of the study given only the scan as input. For $x=\{45, 90, 180, 365\}$ we show AUROC across five different random seeds. We compare three approaches: (teal, left) a single task model pre-trained on Kinetics, (orange, middle) a single task model pre-trained on full-body abnormality detection (in-domain pretraining), and (right, blue) multi-task abnormality \del{localization} \add{detection} model fine-tuned to predict patient's date of death.}  \addc{Confidence intervals ($95\%$) about the mean were determined using bootstrapping across $n=5$ random seeds.}
}\label{fig:multi-task}}
\end{figure}

\clearpage
\thispagestyle{empty}

\begin{figure}
\centering
{\spacing{1}\fontsize{7}{8}\selectfont
\includegraphics[width=\textwidth, height=13.8cm]{FIG/FIG5/figure_5.pdf}
\caption{
\textbf{\added{Spatial attention mechanisms improve automated \del{localization} \add{detection} performance and facilitate model interpretation.}}
%
\textbf{(a)} Models trained with the attention mechanism see a modest improvement over a naive sum reduction, with a 3 point increase in mean AUROC taken over all tasks and all seeds ($p = 0.0002$ paired permutation test, \addc{$n$= 26 tasks evaluated over 5 random seeds}). We show overall performance (far left), as well as performance on a subset of regions. \addc{Confidence intervals ($95\%$) about the mean were determined using bootstrapping across $n=5$ random seeds.}
%
\textbf{(b-c)} The soft-attention mechanism, supervised only by weak abnormality-\del{localization} \add{detection} labels, learns to attend to the appropriate part of the scan. The scan encoder transforms a $2\times224\times224\times200$ PET-CT scan into a $1{,}024\times7\times7\times33$ encoding. The soft-attention mechanism reduces this encoding to a single $1{,}024$-dimensional vector by computing a weighted sum of the voxels in the encoding (see Methods). The opacity of each voxel is proportional to the weight assigned to the voxel by the soft-attention mechanism. 
%We show the attention distributions for (b) the liver, cervical lymph node, right lung and left lung and (c) the carinal, retroperitoneal, supraclavicular and inguinal lymph nodes. 
%
\textbf{(d-g)} Two-dimensional saliency maps facilitate the interpretation of correct \textbf{(d-e)} and incorrect \textbf{(f-g)} abnormality \del{localization} \add{location estimation} predictions. Shown in the first row are FDG-PET uptake values overlaid over CT. FDG-PET values are normalized by subtracting the minimum value in the slice and dividing by the maximum. Additionally, in order to decrease image scatter, we clip PET values at the value of the \nth{60} percentile pixel in the slice. Shown in the second row are saliency maps overlaid over CT. Saliency maps are produced by computing the gradient of the scan model prediction with respect to the input scan and normalizing such that the saliency for each pixel is in the range $[0, 1]$ (See Methods). The color bars for the normalized PET and saliency values are shown in the legend. \textbf{(d)} The model accurately detects a hypermetabolic pulmonary nodule along the medial aspect of the left lung shown in the PET (top). The model's saliency is highly concentrated in the pixels containing the nodule (bottom). \textbf{(e)} A \added{right level II} cervical hypermetabolic lymph node (top) is detected by the scan model. The saliency map is focused precisely on the abnormality (bottom).
%
\textbf{(f)} \added{The model detects abnormal mild FDG uptake in a subcentimeter right inguinal lymph node, around which there is a significant concentration of saliency (bottom panel). However, the clinical report does not mention this finding because, in the context of the patient's cancer, the lymph node is deemed non-specific and likely physiologic or inflammatory. Because the model and the clinical report are not congruent, this is a classified as a false positive, however the model is flagging FDG uptake that at least warrants review.}
\textbf{(g)} The model fails to detect an abnormality in a hypermetabolic left axillary lymph node of a patient with metastatic breast cancer and a pacemaker in the left chest wall (left panel). While the saliency map is concentrated on the abnormal node, the threshold for an abnormal prediction is not reached perhaps because of the the overlying beam hardening artifact from the pacemaker.
}\label{fig:interpretations}}
\end{figure}


==> tables.tex <==
% !TEX root = main.tex

\end{landscape}


